ExplanationLP: Abductive Reasoning for Explainable Science Question Answering

We propose a novel approach for answering and explaining multiple-choice science questions by reasoning on grounding and abstract inference chains. This paper frames question answering as an abductive reasoning problem, constructing plausible explanations for each choice and then selecting the candidate with the best explanation as the final answer. Our system, ExplanationLP, elicits explanations by constructing a weighted graph of relevant facts for each candidate answer and extracting the facts that satisfy certain structural and semantic constraints. To extract the explanations, we employ a linear programming formalism designed to select the optimal subgraph. The graphs' weighting function is composed of a set of parameters, which we fine-tune to optimize answer selection performance. We carry out our experiments on the WorldTree and ARC-Challenge corpus to empirically demonstrate the following conclusions: (1) Grounding-Abstract inference chains provides the semantic control to perform explainable abductive reasoning (2) Efficiency and robustness in learning with a fewer number of parameters by outperforming contemporary explainable and transformer-based approaches in a similar setting (3) Generalisability by outperforming SOTA explainable approaches on general science question sets.

==> sections/evauation_copy.tex <==
% \vspace{-\baselineskip}
\section{Empirical Evaluation}


\paragraph{Background Knowledge for QA} As stated in Section 2, our approach requires two different knowledge bases: Abstract KB and Grounding KB. We construct these knowledge bases using the following corpora.

\noindent\textbf{(1) Abstract KB}: We build our Abstract knowledge base by extracting a selected set of facts from the WorldTree Corpus \cite{jansen2018worldtree}. The corpus provides a knowledge base containing 4,097 common sense and scientific facts to create explanations for multiple-choice science questions. The corpus is built for answering elementary science questions with possible knowledge reuse to elicit explanatory patterns. Each fact in an explanation is assigned a specific role, which represents its function in the explanation: (a) \emph{Central role:} The core sentences that constitute the scientific explanation for a question (e.g., \emph{friction causes the temperature of an object to increases}); (b) \emph{Grounding role:} Sentences connecting abstract terms in a core sentence with concrete terms in the question. This role is usually realized through taxonomic facts (e.g., \emph{a stick is a kind of object}); (c) \emph{Lexical Glue role:} Lexical links between concepts in the sentences to increase the graph connectivity. Synonyms typically represent this role (e.g., \emph{to rub together means to move against}).  In contrast to grounding and lexical glues fact, which are highly coupled with the question, central facts represent the core concept a question is testing, such as actions (\texit{friction occurs when two object’s surfaces move against each other}) or affordances (\texit{friction causes the temperature of an object to increase}). Hence we ignore the grounding and lexical glue facts and build our abstract knowledge base with only central facts. 

\noindent\textbf{(2) Grounding KB}: Grounding knowledge base should consist of synonymous or taxonomic knowledge that can help connect the abstract facts to the question. We use ConceptNet as our grounding facts. ConceptNet has higher coverage and precision, enabling us to answer a wide variety of questions. Our approach does not require \emph{dev-set}, since the possibility of over-fitting is non-existent with only nine parameters.

\noindent\textbf{Question sets}:  We use the following question sets to evaluate our approach's performance and compare it against contemporary neural and explainable approaches. 

\noindent\textbf{(1) WorldTree Corpus}: The 2,290 questions in the WorldTree corpus are split into three different subsets: \emph{train-set} (987), \emph{dev-set} (226), and \emph{test-set} (1,077). We only consider questions with explanations for our evaluation. We use the \emph{dev-set} to assess the explainability performance and error analysis since only \emph{dev-set} has publicly available explanations.

\noindent\textbf{(2) ARC-Challenge Corpus}: ARC-Challenge is a multiple-choice question dataset which consists of question from science exams from grade 3 to grade 9~\cite{clark2018think}. We only consider the Challenge set of questions. These questions have proven to be challenging to answer for other LP-based question answering and neural approaches. We train our approach on the \emph{train-set} (1,119) and test on the \emph{test-set} (1,172). 

\noindent\textbf{Relevant Facts Retrieval (FR)}:
We experiment our approach with two different facts retrieval models. The first model -- i.e. \emph{BM25 Retrieval}, adopts a BM25 vector representation for question, candidate answers and explanation sentences. We apply this BM25 retrieval for Grounding retrieval.
% This representation is used to retrieve the top $k$ candidate facts according to a relevance score computed through the cosine similarity function. 
The second approach -- i.e. \emph{Unification Retrieval (UR)}, represents the BM25 implementation of the Unification-based Reconstruction framework described in \citet{valentino2020unification}. The framework combines the BM25 relevance score with a unification score, representing the fact's explanatory power. Specifically, the unification score for a given fact depends on how often the same fact appears in explanations for similar questions stored in an Explanation KB. This knowledgebase, in line with \citet{valentino2020unification},  is constructed using questions and explanations in the WorldTree train-set. Since the unification retrieval relies on the existence of ExplantionKB, we employ this approach to retrieve abstract facts retrieval with BM25 retrieval for Grounding KB. Unification retrieval has shown to exhibit better performance for retrieving explanatory facts compared to BM25 and transformer-based approaches. 

%while the similarity function between the questions is realized through BM25 vectors and cosine similarity. 
% The Unification Retrieval model has shown better performance when compared to the BM25 Retrieval model in the task of ranking explanatory sentences for multiple-choice science questions.
% , improving the retrieval of complex scientific facts that have low degree of overlaps with question and candidate answer.  

\noindent\textbf{Baselines}: We replicate following the baselines for WorldTree corpus to compare against our approach: 

\noindent \textbf{(1) Bert-Based models}: We compare the ExplanationLP model's performance against a set of BERT baselines. The first baseline -- i.e. \emph{BERT$_{Base}$}/\emph{BERT$_{Large}$}, is represented by a standard BERT language model \cite{devlin2019bert} fine-tuned for multiple-choice question answering. Specifically, the model is trained for binary classification on each question-candidate answer pair to maximize the correct choice (i.e., predict 1) and minimize the wrong choices (i.e., predict 0).  Also, we reproduce two BERT baselines enhanced with explanation sentences retrieved by the retrieval models. The first model \emph{BERT + BM25}  is fine-tuned for binary classification by complementing the question-answer pair with grounding facts and abstract facts selected by BM25 retrieval. Similarly, the second model \emph{BERT + UR} complements the question-answer pair with grounding facts retrieved by BM25 and abstract facts selected by Unification retrieval.

\noindent \textbf{(2) PathNet}~\cite{kundu2018exploiting}: PathNet attempts to extract implicit relations from text through entity pair representations and compose them to encode each path. PathNet is an explainable approach that can explain the reasoning via the explicit reasoning paths. They have exhibited strong performance for multiple-choice science questions and provide a contrast to compare against another graph-based approach. Similar to  BERT-based models, we employ PathNET with the top $k$ facts retrieved via Unification (\emph{PathNet + UR}) and BM25 (\emph{PathNet + BM25}) retrieval. We concatenate the facts retrieved for each candidate answer and provide as supporting facts.

\subsection{Answer Selection}
\setlength{\tabcolsep}{3pt}

\begin{table}[!htb]
    \centering
    \begin{tabular}{@{}cp{3.5cm}cccc@{}}
    \toprule
    \# & \textbf{Model}  & \multicolumn{4}{c}{\textbf{Accuracy}}  \\
    && \textit{k}=20 & \textit{k}=30 & \textit{k}=40 & \textit{k}=50 \\
     \midrule
    \multicolumn{6}{c}{\textbf{Baselines}} \\
    \midrule
    1 & BERT$_{Base}$  & \multicolumn{4}{c}{44.56}\\
    2 & BERT$_{Large}$ & \multicolumn{4}{c}{47.26} \\
    \midrule
     3 & BERT$_{Base}$ + BM25   & 43.63 &37.97 & 31.56 & 32.68   \\
    4 &  BERT$_{Base}$ + UR & 42.14 & 31.84 & 30.36 & 31.29  \\
     5 & BERT$_{Large}$ + BM25 & 43.36 & 32.86 & 35.46 & 26.92 \\
    6 &  BERT$_{Large}$ + UR  & 42.98 & 27.39 & 24.88 & 26.55   \\
     \midrule
      7 & PathNet + BM25  & 41.61 & 41.98 &40.11 & 41.79 \\ 
      8 & PathNet + UR & 43.58 & 40.76 & 41.22& 42.83  \\ 
      \midrule
    \multicolumn{6}{c}{\textbf{ExplanationLP}} \\
    \midrule
    9 & ExplanationLP + BM25  & 50.88 & 50.51 & 50.78 & 50.41  \\ 
    10 & ExplanationLP + UR  &  55.24 &  \underline{\textbf{56.36}} & 54.21 & 54.24 \\ 
     \bottomrule
    \end{tabular}
    \caption{\small Answer selection performance on the WorldTree \emph{test-set}. \textit{k} represents the number of retrieved facts by the respective retrieval approaches.}
    \label{tab:wt_answer_selection_k}
    \centering
    \begin{tabular}{@{}cp{5cm}ccc@{}}
    \toprule
    \# & \textbf{Model} & \multicolumn{2}{c}{\textbf{Accuracy}}  \\
    &&  \textbf{Easy} & \textbf{Challenge} \\
    \midrule
    \multicolumn{4}{c}{\textbf{Baselines}} \\
    \midrule
    11 & BERT$_{Base}$ & 51.04 & 28.75  \\
    12 & BERT$_{Large}$ & 54.58 & 29.39 \\
    \midrule
     13 & BERT$_{Base}$ + BM25 (\textit{k}=20) & 45.54 & 38.97       \\
    14 &  BERT$_{Base}$ + UR (\textit{k}=20)& 44.10 & 37.80  \\
     15 & BERT$_{Large}$ + BM25 (\textit{k}=20) & 45.94 & 37.06   \\
    16 &  BERT$_{Large}$ + UR (\textit{k}=20) & 43.97 & \underline{\textbf{40.57}}    \\
     \midrule
     17 & PathNet + BM25 (\textit{k}=20)  & 43.32 & 36.42   \\ 
      18 & PathNet + UR (\textit{k}=15) & 47.64 & 33.55   \\ 
     \midrule
    \multicolumn{4}{c}{\textbf{ExplanationLP}} \\
    \midrule
    19 & ExplanationLP + BM25 (\textit{k}=20) & 54.49 & 39.61 \\ 
    20 & ExplanationLP + UR (\textit{k=}20) & \underline{\textbf{62.82}} & \underline{\textbf{40.57}} \\ 
     \bottomrule
    \end{tabular}
    \caption{\small Accuracy on Easy and Challenge split of WorldTree corpus from the best performing model}
    \label{tab:wt_answer_selection_split}
\end{table}



\begin{table*}[!htb]
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{@{}cp{9cm}ccP{1.5cm}P{1.5cm}c@{}}
    \toprule
    \# & \textbf{Model} & \textbf{Explainable} &\textbf{Pre-Trained} & \textbf{External \newline KB} & \textbf{Supervised} & \textbf{Accuracy}  \\
    \midrule
    \multicolumn{6}{c}{\textbf{Previous Works (from ARC Leaderboard)}} \\
    \midrule
     1 & TupleInf & Yes & No  & Yes&No & 23.83   \\ 
     2 & TableILP & Yes & No  & Yes&No &  27.11  \\ 
     3 & IR-Solver & Yes & No  & No &No &20.26  \\ 
     4 & DGEM & Partial & No  & Yes & Yes & 27.11 \\

     5 & KG$^2$ & Partial  & Yes & Yes & Yes & 31.70 \\
    %  \midrule
     6 & AHE (FLAIR+BERT) \cite{yadav2019alignment} & Partial & Yes & No  &Yes &33.87 \\ 
     7 & AHE (FLAIR+BERT+GloVe+InferSent) with grade \cite{yadav2019alignment} & Partial & No& No & Yes &\textbf{34.47} \\ 
     8 & Sanity Check & Partial & Partial & No  & Yes & 26.56  \\ 
    % \midrule
    % \multicolumn{6}{c}{\textbf{Baselines}} \\
    % \midrule
    % 5 & BERT$_{Base}$ & N &   50.00 \\
    % 6 & BERT$_{Large}$ & N &  50.00 \\
    % \midrule
    %  7 & BERT$_{Base}$ + BM25 (\textit{k}=) &P &  36.07   \\
    %  8 & BERT$_{Large}$ + BM25 (\textit{k}=25) & P &  43.45  \\
    %  \midrule
    %  9 & PathNet + BM25 (\textit{k}=)  &Y&  65.18   \\ 
    
     \midrule
    \multicolumn{6}{c}{\textbf{ExplanationLP}} \\
    \midrule
    9 & ExplanationLP + BM25 (\textit{k}=20) & Yes & No & Yes & \multirow{ 2}{*}{Minimal} &\textbf{32.16}  \\ 
    10 & ExplanationLP + UR (\textit{k}=30) & Yes & No & Yes & &30.54  \\ 
     \bottomrule
    \end{tabular}}
    \caption{\small ARC challenge scores.}
    \label{tab:arc_answer_selection}
\end{table*}







Table~\ref{tab:wt_answer_selection_k} reports the analyses carried out with BERT, PathNet, and ExplanationLP on the WorldTree \emph{test-set}. We also report the score on the Easy and Challenge subsets for the best model in each category in Table~\ref{tab:wt_answer_selection_split}. We experiment with varying top \textit{k} relevant facts retrieved using fats retrieval. We retrieve top $l$  relevant grounding facts from Grounding KB and top $m$ relevant abstract facts from Abstract KB such that $l + m = k$ and $l:m = 1:1$. 

\noindent We draw the following observations from the table:

\noindent (1) Despite having a smaller number of parameters to train (BERT-base: 110M parameters, BERT-Large: 340M parameters, ExplanationLP: 9 parameters), the best performing ExplanationLP (Row~\#10, \textit{k}=30) overall outperforms both BERT$_{Base}$ and BERT$_{Large}$ with no explanations by 11.8\% (Row~\#1) and  9.1\% respectively. We also outperform BERT with no explanations in both Easy and Challenge split by 8.28 (Row~\#12, Row~\#20) and 11.18 (Row~\#12, Row~\#20), respectively. 

\noindent (2) The lowest drop in performance of our approach with BM25 is 0.46\% (Row~\#9, \textit{k}=20 and \texit{k}=50), and UR is  2.42\% (Row~\#9, \textit{k}=30 and \textit{k}=50). On the other hand, the lowest drop in performance for BERT$_{Large}$ with BM25 is 16.44\% (Row~\#5, \texit{k}=20, and \texit{k}=50), and UR is  16.43\% (Row~\#6, \textit{k}=20 and \textit{k}=50). Similarly, BERT$_{Base}$ with BM25 and UR has the lowest drop of performance of 10.95\% and 10.85\%, respectively. This scores and the overall drop in performance indicates how BERT with explanations struggles with the increasing number of facts as they introduce more noise for the inference. In contrast, our approach can operate on a higher amount of distracting information and still obtain better scores, displaying resilience towards distracting knowledge.

\noindent (3) Similar to our approach, PathNet is explainable and also demonstrates robustness to noise. However, we outperform PathNet's best model by 12.78\% (Row#10, \textit{k}=20 and Row#8, \textit{k}=20). We also outperform PathNet significantly on both Easy and Challenge split (Row~\#17,\#18 and Row~\#19,\#20).  

\noindent (4) We also exhibit better scores on both BM25 and UR compared to BERT and PathNet, demonstrating that our approach is independent of the upstream retrieval in terms of performance.

\noindent (5) BERT, by itself, does not provide any explanations. BERT + Fact Retrieval (FR) is comparatively better since the facts provided by the FR could function as an explanation. However, BERT is still inherently a black-box model, not being entirely possible to explain its prediction. By contrast, ExplanationLP is fully explainable and produces a complete explanatory graph. The model design, by principle, supports full interpretability of the reasoning behind the answer prediction.


\subsection{Explanation Retrieval}
\label{sec:explanation_retrieval}

\begin{table}[h]
    \centering
\begin{tabular}{lcccc}
    \toprule
    \textbf{Approach}  & \multicolumn{4}{c}{\textbf{F1@\textit{k}}}\\
    \cmidrule{2-5}
    & \textit{k=}20 & \textit{k=}30 & \textit{k=}40 & \textit{k=}50 \\
    \midrule
      UR Only & 33.08 & 24.63 & 21.08 & 19.03  \\
      UR + ExplanationLP & 44.00 & 44.07 & 43.88 & 43.88 \\
      \midrule
      BM25 Only  & 24.62 & 20.23  &17.16 & 15.19\\
      BM25 + ExplanationLP  &  36.01 &35.93&35.81&35.81\\
    \bottomrule
    \end{tabular}
    \caption{\small Explanation retrieval performance on the WorldTree Corpus \emph{dev-set}. \textit{k} indicates the number of retrieved facts by the respective retrieval approaches.  }
    \label{tab:explanation_selection}
\end{table}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{images/correct_answer.pdf}
%     \caption{An example of explanations and scores retrieved from ExplanationLP. The answer for this question is \textit{first quarter} which was correctly predicted.}
%     \label{fig:correct_answer}
% \end{figure*}


Table~\ref{tab:explanation_selection} shows the F1 score for explanation retrieval (abstract facts only) of varying number of facts  (\textit{k} facts) retrieved using the FR approaches. As the number of facts increases, the F1 score of FR approaches drops drastically, indicating the increase in distracting knowledge. This stability in performance with the increasing number of distractors adds evidence to our approach's robustness towards the noise and explainability.



% Figure~\ref{fig:correct_answer} illustrates a qualitative example of depicts a set of explanations and scores retrieved by our approach. We can observe for the wrong choices $F_{G2}$ is chosen as a grounding because of the word \textit{picture} in the question (Question-Grounding relevance). This fact, in turn, links to $F_{C1}$ (Grounding-Central inter-hop overlap). For the correct choice, $F_{G5}$ links to a different abstract fact which shares lexical clustered near $F_{C4}$ (Central-Central intra-hop overlap). $F_{C1}$ does not share a lexical overlap with any of the selected abstract facts; hence ExplanationLP avoids selecting this and consequently not select $F_{G2}$ (Abstract fact limit constraint). 

\subsection{Ablation Studies}
\label{sec:ablation}

In order to understand the contribution lent by different components, we choose the best setting (ExplanationLP + UR (\textit{k}=30)) and drop different components to perform an ablation analysis. We retain the ensemble after dropping each component. The results are summarized in Table~\ref{tab:ablation}. 

To understand the impact of grouping facts into grounding and abstract, we drop the grouping and consider all facts as abstract (Row~\#2). Row~\#3 and Row \#4 report the accuracy when all facts are considered to be of the same overlap and relevance score respectively. Row~\#5 and \#6 record the scores in the absence of linear programming constraints. Replacing the abstract fact limit constraint with the maximum number of nodes $K$ would render all solutions infeasible; hence it has not been listed. We set the parameters with a positive domain to 1 and rest to -1. This ablation preserves our initial hypothesis and shows the impact of Bayesian optimization (Row~\#7). 

Table~\ref{tab:hyper} reports the parameters values obtained for the best accuracy score. Unlike contemporary neural approaches, our parameters can be interpreted.

\begin{table}[h]
    \small
    \centering
     \resizebox{\columnwidth}{!}{\begin{tabular}{cp{6cm}c}
    \toprule
    \#& \textbf{Approach} &   \textbf{Acc} \\
    \midrule
    1 & ExplanationLP + UR (\textit{k} = 20) \textbf{(Best)} & \textbf{56.36} \\
    \midrule
    &\multicolumn{2}{l}{\textbf{\underline{Structure}}} \\
    2 & -No Grounding-Abstract Categories &  25.62\\
    \midrule
    &\multicolumn{2}{l}{\textbf{\underline{Score}}} \\
    3 & -No Overlap Score ($O(f_1,f_2) = 1$) & 54.78 \\
    4& -No Relevance score ($R(f) = 1$) & 42.43 \\
    \midrule
      &\multicolumn{2}{l}{\textbf{\underline{ILP Constraints}}} \\
      5&-No Chaining constraint &  41.03  \\
    %   7&-No Abstract fact limit constraint & \\
      6&-No Grounding neighbor constraint & 55.07 \\
    %   7&-No Coverage constraint&  55.07 \\
    \midrule
    7 & -No Parameter tuning & 41.31 \\
    \bottomrule
    \end{tabular}}
    \caption{\small Ablation study, dropping different components of ExplanationLP + UR (\textit{k} = 20). The scores reported here are accuracy for answer selection on the WorldTree development set.}
    \label{tab:ablation}
\end{table}

\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{\begin{tabular}{cp{5.5cm}ccc}
    \toprule
    \textbf{\#} & \textbf{Parameter} & \multicolumn{2}{c}{\textbf{Value}} \\
    &&\textbf{WT} & \textbf{ARC}\\
    \midrule
     8 & Question-Abstract overlap ($\theta_{qa}$) & 0.10 & 0.09 \\
     9 & Question-Grounding overlap ($\theta_{qg}$) & 0.98 & 0.84 \\
     10 & Abstract-Abstract overlap ($\theta_{aa}$) & 0.01 & 0.11 \\
     11 &  Grounding-Abstract overlap ($\theta_{ga}$) & 0.14 & 0.23   \\
     12 & Grounding-Grounding overlap  ($\theta_{gg}$) & -0.99 & -0.92 \\
     \midrule
     13 & Abstract Relevance ($\theta_{ar}$) & 0.03 & 0.09  \\
     14 & Grounding Relevance ($\theta_{gr}$) & 0.36 & 0.14 \\
     \midrule
    %  8 &  Coverage weight ($\theta_{cw}$) & 0.54 & 0.23  \\
     15 &  Edge weight ($\thetha_{ew}$) & 0.80 & 0.26 \\
     16 & Node weight ($\theta_{nw}$) & 0.76 & 0.67 \\
    \bottomrule
    \end{tabular}}
    \caption{Hyperparameters obtained from optimizing  ExplanationLP (best models) for answer selection for ARC and WorldTreeCorpus (WT) and ARC-Challenge (ARC) corpus.}
    \label{tab:hyper}
\end{table}


We draw the following observations from the tables (Table~\ref{tab:ablation},~\ref{tab:hyper}):
% validating our research hypotheses (\textbf{RH}) listed in Section~\ref{sec:construct_graph}:

\noindent (1)  Removing the categorization of grounding-abstract facts lowers the performance by 30.74\% (Row~\#2), showing the impact of grounding-abstract chains in answer selection. 

\noindent (2)  The difference in performance at Row~\#1 and~\#4 (-30.18\%) validates the importance of relevance scores. The high hyperparameter scores obtained for abstract relevance (Row~\#13) and grounding relevance (Row~\#14) corroborate this finding.

\noindent (3)  The performance drop between Row~\#1 and~\#5 (-15.33\%) highlights the importance of chaining constraints. Without the chaining constraint, the LP approach would pick the highest relevance and edges with positive values, ignoring negative edges. If negative edges are not selected, the LP system would not be encouraged to have diverse grounding facts. This observation is also consistent with the grounding-grounding overlap hyperparameter score (Row~\#12).

\noindent (4) The abstract-abstract overlap score (Row~\#8) is relatively smaller, indicating a lower level of importance. However, it still plays a role in the final score, stipulating the need for encouraging conceptual similarity between abstract facts.

\noindent (5) The optimal score we obtain for question-grounding (Row~\#8) and grounding-abstract scores are relatively high. These scores and the drop in performance with no grounding neighbor constraint indicate the importance of grounding facts (Row~\#6) in the final prediction.


\subsection{Error Analysis}
\label{sec:error_analysis}

% We present the error analysis for question answering accuracy.

\noindent\textbf{Explanation Length.} Figure~\ref{fig:explanation_length} plots the change in accuracy as we consider questions with longer explanations. Since our approach was only composed of two hops, we anticipated a loss in performance as the required number of explanations increased. This performance degradation is evident in the graph. Since BERT does not rely on external knowledge, the performance was stable across the spectrum. PathNet also makes two-hop assumptions. However, unlike our approach, they only combine two facts to answer the question. This assumption is evident with higher accuracy for questions with lower explanation length and steep degradation in performance as the explanation length increase.

\noindent\textbf{Entity Overlap between choices.} Figure~\ref{fig:choice_overlap} illustrates the change in accuracy as the entity overlap between answer and other candidate answers increases. In this case, the lexical overlap is calculated as the overlap of unique terms.  Despite our approach dependent on lexical overlaps, there is minimal degradation in performance, indicating that the constraints and structure help alleviate the noise rising from the lexical space. 

\noindent\textbf{Number of Entities in Question and Answer.} Figure~\ref{fig:question_word_count} presents the change in accuracy as the number of entities increases in question and answer. With an increasing number of entities, there are more distractors; thus, a drop in performance is high than PathNet and BERT. This drop can be termed as a limitation of our approach. We believe that rather than treating all entities equally, the scores could be increased by extracting the essential terms.


\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth,height=5cm]{images/exp_len.png}
        \caption{Explanation Length Vs Accuracy}
        \label{fig:explanation_length}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth,height=5cm]{images/histogram.png}
        \caption{Candidate answers entity overlaps Vs Accuracy}
        \label{fig:choice_overlap}
    \end{subfigure}
     ~ 
    % \begin{subfigure}[t]{\columnwidth}
    %     \centering
    %     \includegraphics[width=\columnwidth,height=5cm]{images/concepts.png}
    %     \caption{Unique Concepts Vs Accuracy}
    % \end{subfigure}
     ~ 
    \begin{subfigure}[t]{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth,height=5cm]{images/question_word.png}
        \caption{ Number of Entities in Question Vs Accuracy}
        \label{fig:question_word_count}
    \end{subfigure}
    \caption{\small Quantitative analysis of answer prediction accuracy on the development set varying across different models for WorldTree \emph{dev-set}. Red line represents ExplanationLP + UR (\textit{k}=20), blue line represents BERT$_{Large}$ and  green line represents PathNet + UR (\textit{k}=20)}
\end{figure}

